Towards Robust Benchmarking of Quantum Optimization Algorithms

Benchmarking the performance of quantum optimization algorithms is crucial for identifying utility for industry-relevant use cases. Benchmarking processes vary between optimization applications and depend on user-specified goals. The heuristic nature of quantum algorithms poses challenges, especially when comparing to classical counterparts. A key problem in existing benchmarking frameworks is the lack of equal effort in optimizing for the best quantum and, respectively, classical approaches. This paper presents a comprehensive set of guidelines comprising universal steps towards fair benchmarks. We discuss (1) application-specific algorithm choice, ensuring every solver is provided with the most fitting mathematical formulation of a problem; (2) the selection of benchmark data, including hard instances and real-world samples; (3) the choice of a suitable holistic figure of merit, like time-to-solution or solution quality within time constraints; and (4) equitable hyperparameter training to eliminate bias towards a particular method. The proposed guidelines are tested across three benchmarking scenarios, utilizing the Max-Cut (MC) and Travelling Salesperson Problem (TSP). The benchmarks employ classical mathematical algorithms, such as Branch-and-Cut (BNC) solvers, classical heuristics, Quantum Annealing (QA), and the Quantum Approximate Optimization Algorithm (QAOA).

==> txt/3_Related-Work.tex <==
%See comments for sketch of the planned content

%List of classical and quantum benchmarking frameworks (steal from ~\cite{lubinski2024optimization})
%Much background material is available on benchmarking classical solutions to optimization problems [3, 62 , 77 ] and comparing quantum methods to classical solutions [ 78 – 80 ]

%Benchmark frameworks such as SupermarQ [67 ] and QPack Scores [ 68] include one or more QAOA applications in their sample benchmarks, while QUARK [ 69] considers specific optimization problems arising in industry.

%and of course: Benchmarking Framework for QAOA and QA (D-Wave Paper)~\cite{lubinski2024optimization}
%QED-C (https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=10061574)
%Benchmakring when hardware can execute wihich standard algorithms, while investigating: #Qubits, Circuitdepth, and outputfidelity

%then https://arxiv.org/pdf/2302.02278.pdf adapted QED-C for optimization specific problems/algorithms -> TTS (Time to solution) and TTT (Time to target [quality threshold ... of the solution])

%in general the QED-C stuff is very much problem instance unaware and therefore not specific enough if one want to find the best classical and quantum approaches to solve the problem, it simply compares the standard existing classical and quantum approaches (no specialization what so ever) ... in contrast to our approach.

%Paper on Quantum Optimization in general, including a large section on best- practices for benchmarking~\cite{abbas2023quantum}%tbc... (sorry, got no time)

%QAOA (and QA) on MaxCut eval (incl. somewhat efficient approach to optimize QAOA parameters for MaxCut)~\cite{PhysRevX.10.021067}

%Evaluation of Max-Cut heuristics~\cite{doi:10.1287/ijoc.2017.0798}

%(QML benchmarking is different than ML benchmarking~\cite{bowles2024better})

%(Benchmarking hybrid solvers~\cite{Oshiyama2022})

==> txt/5_Examples/03_mc_scenario3.tex <==

\subsubsection{Scenario 3}

% \paragraph{Goal} Solve real-world problems that are economically relevant and the best solution can not be found by state of the art. Probably consider one specific domain, e.g. which Algorithm should a chip company use to build the best chip?

% \paragraph{Restrictions} Many algorithms can not be used due to infeasible runtimes.

% \paragraph{Suitable dataset} Graphs that are related to real-world problems and very difficult to solve. More than 1000 variables and high connectivity.

% \paragraph{Metric} Solution Quality within the time limit.

% \paragraph{Algorithms} GW, SA, Tabu, QA?, DA?

% \paragraph{Hyperparameter tuning} Manual or intuitive selection as problems need hours to solve.

% \paragraph{Analysis} Compare different time limits on different problems. Clear recommendation which algorithm should be used in production.

In the third scenario, we aim to assess the effectiveness of solving large, real-world MC instances. All algorithms are executed with a time limit of 60 seconds.

\paragraph{Algorithms} We consider the same algorithms as used in the second scenario, except DW, as the instance sizes from the dataset exceed the current hardware capabilities.

\paragraph{Dataset} The chosen dataset addresses VLSI instances consisting 522--4640 nodes with 906--8255 edges form MQLib~\cite{dunning_what_2018}. This dataset is split into two subsets. The first subset contains 68 instances with 522--987 nodes and 906--1923 edeges and the second subset 72 instances with 1005--4640 and 1731--8255 edges. This split is required as the community edition of CPLEX is limited to a maximum of 1000 variables. In total, the dataset comprises 140 instances. 

% for the MaxCut use case aims to examine problems that represent real-world examples as closely as possible. To achieve this objective, we utilize problems from the MQLib paper and filter these problems to ensure they have between 500 and 5000 nodes. Furthermore, we exclusively focus on problems that address the arrangement on a VLSI chip.

\paragraph{Figure of Merit} For the same reason as in scenario 2, we use BSF as the figure of merit here.

% Given that we can no longer always guarantee finding the absolute best solution for these problems, we opt for the best solution achievable within a set timeout as our metric. This best solution is then presented as a relative cut size compared to the best solution all algorithms could find for the given problem. It is important to note, that Gurobi often stops before reaching the timeout, which is a benefit not considered in the following comparison.

\paragraph{Hyperparameter tuning} We do not conduct a hyperparameter optimization and use the parameters from the second scenario.

% For Simulated Annealing, we examined the num sweeps hyperparameter. An increased number of num sweeps leads to improved solutions but also results in fewer iterations of the Simulated Annealing process before reaching the timeout. Gurobi was executed without any parameter adjustments.

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{gfx/mc_large_relative_cut_size_err.pdf}
%     \caption{Relative error in cut size for large MC instances within a group}
%     \label{fig:maxcutlargerelcut}
% \end{figure}

% The results indicate that Simulated Annealing achieves better outcomes with a higher number of num sweeps, despite undergoing fewer iterations (see Figure \ref{fig:maxcutlargerelcut}). Furthermore, we observe that for most results, several algorithms have identified the same best solution, suggesting it may already be the optimal solution. Thus both Gurobi and instances of Simulated Annealing with a greater number of num sweeps were able to completely solve the problem. Given that Gurobi often found the solution before reaching the absolute timeout, we speculate that Gurobi may be the most efficient solver for this class of problems.

\paragraph{Results} For the smaller subset, both Gurobi and CPLEX exhibit a relative error of 0.0 for all instances, demonstrating their ability to ascertain the optimal solution in every scenario. Within the second subset, Gurobi maintains a relative error of 0.0 for all instances, confirming its efficacy in identifying the optimal solution for all but one instance\footnote{Gurobi could not verify that its solution is optimal within the set time limit of 60 s.}. The relative error for SA, TS, and Greedy, illustrated in Fig.~\ref{fig:maxcutlargerelcut}, reveals that SA outperforms TS and Greedy, consistently yielding the lowest relative error with the narrowest spread. While TS demonstrates performance comparable to SA for instances with fewer than 876 nodes, its error rate significantly escalates for larger instances. Conversely, Greedy underperforms across all instances, incurring the highest relative errors and exhibiting the greatest variability.
% In contrast to the second scenario the relative error for SA decreases with an increasing number of nodes, 

\begin{figure}
\centering
\includegraphics[width=0.9\linewidth]{gfx/mc_large_relative_cut_size_err.pdf}
\caption{Relative error in cut size for large MC instances within a group.}
\label{fig:maxcutlargerelcut}
\end{figure}

